High-Performance Model Predictive Control for Quadcopters with Formal Stability Guarantees

In this paper, we present a novel cascade control structure with formal guarantees of uniform almost global asymptotic stability for the state tracking error dynamics of a quadcopter. The proposed approach features a model predictive control strategy for the outer loop, explicitly accounting for the non-zero total thrust constraint. The outer-loop controller generates an acceleration reference, which is then converted into attitude, angular velocity and acceleration references, subsequently tracked by a nonlinear inner-loop controller. The proposed cascade control strategy is validated through numerical case studies, underlying high-fidelity models, demonstrating its ability to track fast trajectories with small error.

==> Sections/Section11.tex <==
 \vspace{-0.3cm}
 The proposed outer-loop controller, labeled \enquote*{\textit{Proposed MPC}} and detailed in Section \ref{MPC1 Section}, is experimentally evaluated in Europe's largest indoor drone cage---the 20-meter-high Avular drone cage--- using Vertex One quadcopter, as shown in Fig. \ref{drone cage and hovering}. For these tests, a PID-based attitude controller was used as the inner-loop controller.
\begin{figure}[!h]
\centering
\subfloat[]{\includegraphics[width=1.5in,height=2in]{Figures/Drone cage.png}%
\label{drone cage}}
\hfil
\subfloat[]{\includegraphics[width=1.5in,height=2in]{Figures/hovering.jpg}%
\label{hovering}}
\caption{(a) Avular drone cage providing a secure environment for experimental testing. (b) Instance of the Vertex One quadcopter at hovering
position with the \textit{Proposed MPC} in the Avular drone cage.}
\label{drone cage and hovering}
\end{figure}

The Vertex One flight controller is operated by the Real-Time MCU, known as Avular Prime (ARM Cortex-M7), which connects all hardware components of the Vertex One, including propulsion and sensors.
The Vertex One is also equipped with an onboard computing module based on the Nvidia Jetson Xavier NX, providing the ROS 2 wrapper
for the Intel RealSense depth camera. The onboard computing module communicates with the flight controller in Prime via UART.
Due to the hardware limitations of the Prime, the \textit{Proposed MPC} algorithm is implemented on the onboard computing module using the Robot Operating System (ROS), while the MCU handles other control components, including attitude controller. For this setup, the Prime transmits MPC inputs to the Jetson and receives the corresponding MPC outputs. Three MPC nodes for the $x,y$ and $z$ directions are implemented in C++ within the Jetson's user-container, leveraging C++ for its compatibility with the CasADi toolbox. We integrate the CasADi-generated C++ MPC functions into the ROS package by linking against the corresponding header files that declare these functions. The lab experiments are conducted with a sampling time of $h=0.1$ seconds, a prediction horizon $N=10$, a state cost matrix $Q=\mathrm{diag}(10,1,1,1)$, and an input cost matrix $R=1$. The experiment run for a total duration of 20 seconds, using the following reference trajectory:
\begin{align}
\begin{split}
    \Bar{p}(t)&=[p_x(0)+\cos(0.2\pi t),~ p_y(0)+\sin(0.2\pi t),\\ &~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~p_z(0)-1]^{\T}, \notag
   \end{split}\\
\Bar{\psi}(t)&=0.
\label{experiment reference trajectory }
\end{align}
Fig. \ref{trajectory MPC exp} and Fig. \ref{refftrack MPC exp} show the experimental position trajectories alongside the reference trajectory, using the \textit{Proposed MPC} as the outer-loop controller and a PID-based attitude controller in the inner loop. These results demonstrate the effectiveness of the proposed controller in tracking the reference with small error. In Fig. \ref{trajectory PID exp} and Fig. \ref{refftrack PID exp}, the resulting trajectories from using the cascade PID-based controller are presented. Comparison of the trajectory plots from both cases clearly illustrates the MPC controller's ability to reduce overshoot during step changes. This is further confirmed by the RMSE comparison in the $z$ direction, where the RMSE for the \textit{Proposed MPC} and \textit{PID} are \unit{[0.25, 0.12, 0.23]}[m] and \unit{[0.22, 0.09, 0.32]}[m], respectively. It is evident that the \textit{Proposed MPC} significantly outperforms PID in the $z$ direction, while PID achieves smaller errors in the $x$ and $y$ directions.
\begin{figure}
\centering
% Top row
\subfloat[]{\includegraphics[width=0.23\textwidth]{Figures/trajectory_MPC_exp.png}%
\label{trajectory MPC exp}}
\hfil
\subfloat[]{\includegraphics[width=0.23\textwidth]{Figures/refftrack_MPC_exp.png}%
\label{refftrack MPC exp}}
\\ % Line break for the second row
% Bottom row
\subfloat[]{\includegraphics[width=0.23\textwidth]{Figures/trajectory_PID_exp.png}%
\label{trajectory PID exp}}
\hfil
\subfloat[]{\includegraphics[width=0.23\textwidth]{Figures/refftrack_pid_exp.png}%
\label{refftrack PID exp}}

\caption{Experimental trajectory tracking results: (a) and (b) 3D plot and time-series of the reference and actual trajectories using the \textit{Proposed MPC} controller in the outer loop and a PID-based inner-loop controller; (c) and (d) 3D plot and time-series using a PID-based cascade controller. The reference trajectory is shown in red in all figures.}
\label{exp result}
\end{figure}
\begin{figure}[!t]
\centering
\includegraphics[width=2.2in]{Figures/thrust_exp.png}
\caption{Resulting control thrust $T$ and maximum thrust $T_{\mathrm{max}}$ during the first 10 seconds of the experiment.}
\label{thrust exp}
\end{figure}

Fig. \ref{thrust exp} compares the thrust for both cases. While the thrust remains below the maximum value and satisfies constraint (\ref{constraint}) in both cases, the PID thrust plot shows a high initial peak that causes overshoot. The thrust plot also reveals that the \textit{Proposed MPC} delivers a smoother control thrust compared to the noisy thrust from the \textit{PID}, highlighting the effectiveness of the \textit{Proposed MPC} in providing greater reliability.
%and reducing wear and tear on mechanical components.

As demonstrated in all experimental result plots, the controller performed as expected based on the simulation study, and the quadcopter successfully converged to the reference trajectory in this real system experiment. However, in the simulation, \textit{Proposed MPC} outperforms \textit{PID} in the $x$ and $y$ directions, whereas in the experiment, \textit{PID} achieves better results in these directions. One explanation is that the MPC horizon in simulation is set to $N=20$, while in the experiment, it is $N=10$. Another key difference is that the simulation uses the nonlinear controller in the inner loop, while the experiment employs the PID-based attitude controller, with the nonlinear controller potentially outperforming the PID-based attitude controller. The difference could also stem from model inaccuracies.


==> Sections/Section5-2.tex <==
%\vspace{-0.2cm}
\subsection{Algorithm Overview}\label{sec:sec5.2}
\vspace{-0.2cm}
The iterative algorithm to synthesize a DTCBF-triple $(h, \gamma, \pi)$ for the system \eqref{eq:dynamial-sysem-control-affine} with the control admissibe set $\mathbb{U}$ is proposed as follows:
\begin{enumerate}[listparindent=\parindent, label=\textbf{Step \arabic*)}, ref=\arabic*, wide=0pt] \addtocounter{enumi}{-1}
    \vspace{0.2cm}
    \item \textbf{Initialization:}  \label{step:step0} We parameterize $h$, $\gamma$, and $\pi$ as in \eqref{eq:sec4:parameterized-DTCBF}--\eqref{eq:sec4:parameterized-control-policy}, respectively. We also set the degree of auxiliary polynomials  $\widetilde{\pi}_{p,q} \in \mathbb{R}[x]$, $p \in \{1,2, \hdots, m\}$, \mbox{$q \in \{p,p+1, \hdots, m\}$}. We set the degree of SOS multipliers $\Lambda, \Omega, \Phi, \sigma_{p,1}, \hdots, \sigma_{p,4} \in \mathrm{SOS}[x]$, \mbox{$p \in \{1,2, \hdots, m\}$}, $\Psi \hspace{-0.02cm} \in \hspace{-0.02cm} \mathrm{SOS}[x]^{n_U}$, $\xi_{i,j,1}, \hdots, \xi_{i,j,8}, \eta_{i,j,1},\hdots, \eta_{i,j, 8} \in \mathrm{SOS}[x]$, and $\Theta_{i,j,1}, \Theta_{i,j,2}, \Theta_{i,j,3}, \Delta_{i,j,1},\Delta_{i,j,2},\Delta_{i,j,3} \in \mathbb{R}[x]$, \mbox{$i \in \{1,2, \hdots, m-1\}$} and $j \in \{i+1,i+2, \hdots, m\}$. \vspace{0.2cm} \\
We initialize the DTCBF $h^{(0)}$. The polynomial $h^{(0)}$ must be a valid DTCBF, but it can be quite conservative. For example, if the origin is a stable fixed point, a small region around it can be considered.
%can be quite conservative such as a relatively small region around the origin. 
We set the iteration counter to $k\defeq1$.
%\vspace{0.35cm}
%\begin{rem}
%    If the SOS programming problem \eqref{eq:step1:opti1} below becomes infeasible for the initial DTCBF $h^{(0)}$, different initial DTCBFs, such as more conservative ones, can be explored until feasibility is achieved.
    %one can explore different initial DTCBFs, such as using a small circle positioned in different locations.
    %If finding an initial guess for $h^{(0)}$ proves challenging, one can explore different initial DTCBFs (e.g., using a small circle and placing it at various locations). %and observe where they can begin growing.
%\end{rem}
\vspace{0.5cm}
\item \textbf{Updating the Control Policy:} \label{step:step1} Based on Theorem \ref{theorem:sec5:thm1} and given $h^{(k-1)}$ obtained at the $(k-1)$-th iteration, we construct a feasibility problem in SOS programming to update $\gamma$ and its friend $\pi$ as %\vspace{-0.2cm}
\begin{subequations} \label{eq:step1:opti1}
\begin{align}
    \mathrm{find} ~&~ \gamma, \pi_p, \widetilde{\pi}_{p,q}, \Lambda, \Psi, \sigma_{p,1}, \hdots, \sigma_{p,4}, \nonumber \\
    &~\xi_{i,j,1}, \hdots, \xi_{i,j,8}, \eta_{i,j,1}, \hdots, \eta_{i,j,8}, \nonumber \\
    &~\Theta_{i,j,1}, \Theta_{i,j,2}, \Theta_{i,j,3}, \Delta_{i,j,1}, \Delta_{i,j,2}, \Delta_{i,j,3} \\
    \mathrm{s.t.} ~&~ \eqref{eq:sec5:updating_CBF_cons_2}, \eqref{eq:sec5:updating_CBF_modified_function}, \eqref{eq:prop:bi-A-1}, \eqref{eq:prop:bi-A-2}, \eqref{eq:prop:bi-B-1}\textrm{--}\eqref{eq:prop:bi-B-8}, \nonumber \\
    & \gamma, \pi_p, \widetilde{\pi}_{p,q},\Theta_{i,j,1}, \Theta_{i,j,2}, \Theta_{i,j,3}, \nonumber\\
    & \hspace{1.55cm} \Delta_{i,j,1}, \Delta_{i,j,2}, \Delta_{i,j,3} \in \mathbb{R}[x], \\
    &~ \Lambda, \sigma_{p,1}, \hdots, \sigma_{p,4}, \xi_{i,j,1}, \hdots, \xi_{i,j,8}, \nonumber \\
    & \hspace{2.172cm} \eta_{i,j,1}, \hdots, \eta_{i,j,8} \in \mathrm{SOS}[x], \\
    &\hspace{4.1cm} \Psi \in \mathrm{SOS}[x]^{n_U},
\end{align}
\end{subequations}
where $p\in \{1,2, \hdots, m\}$, $q \in \{p,p+1, \hdots, m\}$, \mbox{$i \in \{1,2, \hdots, m-1\}$}, and \mbox{$j \in \{i+1,i+2, \hdots, m\}$}. \vspace{0.3cm}
%\begin{rem}
%    A desired $\gamma$ can be set as an objective of the optimization problem \eqref{eq:step1:opti1}.
%\end{rem}
%\vspace{0.3cm}

Using $\gamma^{(k)}$ and $\pi^{(k)}$ obtained in \eqref{eq:step1:opti1} at the current iteration $k$, we aim to find \mbox{a SOS multiplier $\Omega \in \mathrm{SOS}[x]$} such that \eqref{eq:sec5:updating_CBF_original_function} holds. This multiplier is
essential for updating the DTCBF in the subsequent step. To find it, we construct a feasibility problem in SOS programming as
\begin{subequations} \label{eq:step1:opti2}
\begin{align}
    \mathrm{find} ~&~ \Omega \\
    \mathrm{s.t.} ~&~ h^{(k-1)}(f(x) + g(x)\pi^{(k)}(x)) - h^{(k-1)}(x) + \nonumber \\
    & \gamma^{(k)}(h^{(k-1)}(x)) - \Omega(x) h^{(k-1)}(x) \in \mathrm{SOS}[x], \\
    &\hspace{4.64cm} \Omega \in \mathrm{SOS}[x].
\end{align}
\end{subequations}
%where $\gamma^{(k)}$ and $\pi^{(k)}$ are the solutions of \eqref{eq:step1:opti1} at the current iteration $k$.
%\vspace{0.2cm}
\item \textbf{Updating the DTCBF:} \label{step:step2}
In this step, we obtain the updated DTCBF $h^{(k)}$ by solving the feasibility problem %\vspace{-0.5cm} %To update the DTCBF $h^{(k)}$, we solve the feasibility problem
\begin{subequations} \label{eq:step2:opti1}
\begin{align}
    %&\hspace{-5cm} \mathrm{max}  ~~ \delta \\
    &\hspace{-5cm} \mathrm{find} ~~ h, \Phi, \Xi \\%, \Theta_{i,j,1}, \Theta_{i,j,2}, \Theta_{i,j,3}, \nonumber \\
    %&\hspace{-4.25cm}\Delta_{i,j,1}, \Delta_{i,j,2}, \Delta_{i,j,3} \label{eq:step2:opti1-obj} \\
    \mathrm{s.t.} ~~ \eqref{eq:sec5:updating_CBF_modified_function}, \eqref{eq:prop:bi-A-1}, \eqref{eq:prop:bi-A-2}, \eqref{eq:prop:bi-B-1}\textrm{--}\eqref{eq:prop:bi-B-8}, \hspace{0.5cm}  \nonumber \\
    h(f(x) + g(x) \pi^{(k)}(x)) - h(x&)  +  \nonumber \\
    \qquad \gamma^{(k)}(h(x)) - \Omega^{(k)}(x)h(x) &\in \mathrm{SOS}[x], \label{eq:step2:opti1-const-1} \\
    M\pi^{(k)}(x) + d - \Psi^{(k)}(x)h(x) &\in \mathrm{SOS}[x]^{n_U}, \label{eq:step2:opti1-const-3} \\
    -h(x) - \epsilon + \Phi(x)s(x) &\in \mathrm{SOS}[x], \label{eq:step2:opti1-const-2} \\
    h(x) - \delta - \Xi(x) h^{(k-1)}(x) &\in \mathrm{SOS}[x], \label{eq:step2:opti1-const-4} \\
    \Phi, \Xi &\in \mathrm{SOS}[x], \label{eq:step2:opti1-const-5} \\
    h%, \Theta_{i,j,1}, \Theta_{i,j,2}, \Theta_{i,j,3}, & \nonumber \\
    %\Delta_{i,j,1}, \Delta_{i,j,2}, \Delta_{i,j,3} 
    &\in \mathbb{R}[x].
\end{align}
\end{subequations}
%where \mbox{$i \in \{1,2, \hdots, m-1\}$}, and $j \in \{i+1, i+2, \hdots, m\}$. 
Here, \mbox{$\epsilon, \delta \in \mathbb{R}_{>0}$} are predefined and sufficiently small, $M \in \mathbb{R}^{n_U \times m}$ and $d \in \mathbb{R}^{n_U}$ are associated with the control admissible set $\mathbb{U}$ as in \eqref{eq4:sec4:control-admissible-assumption}, and the mapping $s$ is associated with the safe set $\mathcal{S}$ as in \eqref{eq:sec2:safe-set}. Additionally, $\pi^{(k)}$, $\gamma^{(k)}$, and $\Psi^{(k)}$ are the solutions of the feasibility \mbox{problem \eqref{eq:step1:opti1}}, and $\Omega^{(k)}$ is the solution of the \mbox{problem \eqref{eq:step1:opti2}} at the current iteration $k$. Moreover, $h^{(k-1)}$ is the solution of \eqref{eq:step2:opti1} at the previous iteration.
\vspace{0.35cm}
\begin{rem} \label{rem:sec5:lossless}
    We impose the SOS constraints \eqref{eq:sec5:updating_CBF_modified_function}, \eqref{eq:prop:bi-A-1}, \eqref{eq:prop:bi-A-2}, \eqref{eq:prop:bi-B-1}\textrm{--}\eqref{eq:prop:bi-B-8} in the feasibility problem \eqref{eq:step2:opti1} to ensure that the problem \eqref{eq:step1:opti1} is feasible in the next iteration.
    %Regarding the SOS constraints \eqref{eq:sec5:updating_CBF_modified_function}, \eqref{eq:prop:bi-A-1}, \eqref{eq:prop:bi-A-2}, \eqref{eq:prop:bi-B-1}\textrm{--}\eqref{eq:prop:bi-B-8} in the optimization problem \eqref{eq:step2:opti1}, the SOS multipliers %$\sigma^{(k)}_{p,1}, \hdots, \sigma^{(k)}_{p,4}, \xi_{i,j,1}, \hdots, \xi_{i,j,8}, \eta_{i,j,1}, \hdots,$ $\eta_{i,j,8} \in \mathrm{SOS}[x]$, $p \in \{1,2, \hdots, m\}$, \mbox{$i \in \{1, 2, \hdots, m-1\}$}, $j \in \{i+1,i+2, \hdots, m\}$, 
    In these constraints, the SOS multipliers are fixed and obtained in \eqref{eq:step1:opti1} at the current iteration $k$, 
    while \mbox{$h, a_{i,j} \in \mathbb{R}[x]$}, $i \in \{1,2, \hdots, m\}$, \mbox{$j \in \{i,i+1, \hdots, m\}$}, are unknown. However, we do not restate the constraints to avoid redundancy.
\end{rem}
\vspace{0.35cm}
% \vspace{0.3cm}\\
%the size of $\mathcal{C}^{(k)}$ is larger than the size of the zero-superlevel set $\mathcal{C}^{(k-1)}$ of $h^{(k-1)}$. \vspace{0.3cm}\\ 
%If the optimization problem \eqref{eq:step2:opti1} is feasible, 
If the problem \eqref{eq:step2:opti1} is feasible, we proceed to \mbox{Step \ref{step:step1}} and set \mbox{$k \defeq k +1$}. If it is infeasible, indicating that the size of the zero-superlevel set of the DTCBF can no longer be enlarged, the algorithm is terminated, and we report $(h^{(k-1)}, \gamma^{(k-1)},\pi^{(k-1)})$ as the synthesized DTCBF-triple.

%If $\delta > \delta_0$, where $\delta_0 \in \mathbb{R}_{\geqslant 0}$ is predefined, we proceed to \mbox{Step \ref{step:step1}} and set \mbox{$k \defeq k +1$}. Otherwise, the algorithm is terminated, and report $(h^{(k)}, \gamma^{(k)},\pi^{(k)})$ as the synthesized DTCBF-triple.
%report $h^{(k)}$ as the synthesized DTCBF, and report $\gamma^{(k)}$ and the corresponding control policy $\pi^{(k)}$.
\end{enumerate}

%\begin{rem}
    %It is important to note that our synthesis algorithm does not guarantee that $\gamma^{(1)}$ and $\pi^{(1)}$ can be found for any initial DTCBF $h^{(0)}$ due to the fact that the conditions in \mbox{Step \ref{step:step1}} are sufficient, not necessary. Despite this, the algorithm is \textit{lossless}, meaning that once the conditions in \mbox{Step \ref{step:step1}} are satisfied in the first iteration, their satisfaction in subsequent iterations is guaranteed (see Remark \ref{rem:sec5:lossless}). Moreover, it is guaranteed that $(h^{(l)}, \gamma^{(l)}, \pi^{(l)})$, for all \mbox{$l \in [1, ~k-1] \subset \mathbb{N}$}, forms a DTCBF-triple, and \mbox{$\mathcal{C}^{(l-1)}  \subset \mathcal{C}^{(l)}$}. 
    %if $\gamma^{(0)}$ and $\pi^{(0)}$ are found, the conditions in Step \ref{step:step1} becomes necessary, since the updated DTCBF is constructed in Step \ref{step:step2} in such a way that these sufficient conditions become necessary.
    %convergence to a valid DTCBF. This limitation is also present in almost all existing works on the synthesis of continuous-time CBFs using SOS programming \cite{Ames2019a, dai2022, clark2022, Wang2023b}. However, if $\pi^{(0)}$ and $\gamma^{(0)}$ are obtained for the initial DTCBF $h^{(0)}$, it is guaranteed that $(h^{(l)}, \gamma^{(l)}, \pi^{(l)})$, for all $l \in [1, ~k-1] \subset \mathbb{N}$, is a DTCBF-triple, and $\mathcal{C}^{(l-1)} \subseteq \mathcal{C}^{(l)}$.
    %In our method, this limitation arises due to two key factors. Firstly, \mbox{Theorem \ref{theorem:sec5:thm1}} asserts that if certain conditions are met, the updated control policy is valid. However, the converse statement is not necessarily true. Secondly, similar to existing works on the synthesis of continuous-time CBFs, we utilize the generalized S-procedure lemma (Lemma \ref{lemma:sec4:S-procedure}), which is a sufficient but not necessary condition, and utilize an alternating-descent approach that does not provide convergence guarantees to a valid DTCBF. %However, in Section \ref{sec:sec6}, we will show 
    %that the proposed method can computationally efficiently synthesize DTCBFs.  
%\end{rem}


\begin{thm}
    %If $\pi^{(1)}$ and $\gamma^{(1)}$ can be found for the initial DTCBF $h^{(0)}$ in Step \ref{step:step1} of the proposed algorithm at the first iteration, then it is guaranteed that for each $h^{(l)}$, where $l \in [1, ~k-1] \subset \mathbb{N}$, $\pi^{(l+1)}$ and $\gamma^{(l+1)}$ can be found such that $(h^{(l)}, \gamma^{(l+1)}, \pi^{(l+1)})$ forms a DTCBF-triple, and \mbox{$\mathcal{C}^{(l-1)}  \subset \mathcal{C}^{(l)}$}. 
    The proposed algorithm is lossless, meaning that once the conditions in Step \ref{step:step1} are satisfied, i.e., the control policy $\pi^{(1)}$ and $\gamma^{(1)}$ are found for the initial DTCBF $h^{(0)}$ corresponding to the system \eqref{eq:dynamial-sysem-control-affine} with the control admissible set $\mathbb{U}$, the satisfaction of all conditions is guaranteed, except \eqref{eq:step2:opti1-const-4}, which indicates that the size of the zero-superlevel set of $h$ can no longer be enlarged. Moreover, it is guaranteed that $(h^{(l)}, \gamma^{(l)}, \pi^{(l)})$, for all \hspace{0.05cm}\mbox{$l \in [1, k-1] \subset \mathbb{N}$}, forms a DTCBF-triple for the \mbox{system \eqref{eq:dynamial-sysem-control-affine}} with $\mathbb{U}$, and \mbox{$\mathcal{C}^{(l-1)} \subset \mathcal{C}^{(l)} \subseteq \mathcal{S}$}. %where $\mathcal{S}$ is the safe set as in \eqref{eq:sec2:safe-set}, and $\mathcal{C}^{(l-1)}$ and $\mathcal{C}^{(l)}$ are the zero-superlevel set of $h^{(l-1)}$ and $h^{(l)}$, respectively.
\end{thm}
\vspace{-0.4cm}
\begin{pf}
    Imposing the conditions \eqref{eq:sec5:updating_CBF_modified_function}, \eqref{eq:prop:bi-A-1}, \eqref{eq:prop:bi-A-2}, \eqref{eq:prop:bi-B-1}\textrm{--}\eqref{eq:prop:bi-B-8}, and \eqref{eq:step2:opti1-const-3} in the feasibility problem \eqref{eq:step2:opti1} in Step \ref{step:step2} at the $k$-th iteration, $k \in \mathbb{N}$, ensures that
    all conditions of the problem \eqref{eq:step1:opti1} in Step \ref{step:step1} at the $(k+1)$-th iteration can be satisfied, even in the worst case, with $\pi^{(k)}$ and $\gamma^{(k)}$ obtained at the previous iteration. Subsequently, the feasibility of the \mbox{problem \eqref{eq:step1:opti1}} at the $k$-th iteration, $k \in \mathbb{N}$, guarantees that all conditions of \mbox{Step \ref{step:step2}}, except \eqref{eq:step2:opti1-const-4}, at this iteration can be satisfied with $h^{(k-1)}$. Therefore, the only condition that may halt the algorithm is if the size of the zero-superlevel set of $h$ can no longer be enlarged.
    %if \eqref{eq:step2:opti1} is feasible, then $h^{(l)}$, $l \in \mathbb{N}$, is obtained in such a way that $\pi^{(l+1)}$ and $\gamma^{(l+1)}$ are guaranteed to be obtained at the next iteration. 
    Additionally, based on Lemma \ref{lemma:sec4:S-procedure}, the satisfaction of \eqref{eq:step2:opti1-const-1} and \eqref{eq:step2:opti1-const-3} implies that $(h^{(l)}, \gamma^{(l)}, \pi^{(l)})$, for all $l \in [1, k-1] \subset \mathbb{N}$ is a DTCBF-triple. Lastly, we impose \eqref{eq:step2:opti1-const-2} and \eqref{eq:step2:opti1-const-4} to ensure that $\mathcal{C}^{(l-1)} \subset \mathcal{C}^{(l)} \subseteq \mathcal{S}$. \qed
    %The satisfaction of \eqref{eq:step2:opti1-const-2} implies that the zero-superlevel set $\mathcal{C}^{(l)}$ of $h^{(l)}$ is a subset of the safe set. Lastly, we impose \eqref{eq:step2:opti1-const-4} to ensure that $\mathcal{C}^{(l-1)} \subset \mathcal{C}^{(l)}$, where $\mathcal{C}^{(l-1)}$ is \mbox{the zero-superlevel set of $h^{(l-1)}$}. \qed
\end{pf}



==> Sections/Section6-Ex1-old.tex <==
By discretizing the continuous-time linear system discussed in \cite{Wang2023b} using the zero-order hold method with sampling time $T_s = \unit[1]{s}$, we consider the discrete-time system
\begin{align} \label{eq:sec6:linear-system}
    \begin{bmatrix}
        x^+_{1} \\ x^+_{2}
    \end{bmatrix} = \underbrace{\begin{bmatrix}
        17.6 & 7.3 \\
        22.0 & 10.3
    \end{bmatrix}}_{A}\begin{bmatrix}
        x_{1} \\ x_{2}
    \end{bmatrix} + \underbrace{\begin{bmatrix}
        5.4 & 2.0 \\
        5.9 & 3.4
    \end{bmatrix}}_{B} \begin{bmatrix}
        u_{1} \\ u_{2}
    \end{bmatrix},
\end{align}
where $u_1 \in [-2.5, ~ 2.5]$ and $u_2 \in [-2.5, ~ 2.5]$.
In this example, the safe set is defined as 
\begin{align} \label{eq:sec6:safe-set}
    \mathcal{S} \defeq \{x \in \mathbb{R}^2 \mid x_1^2 + x_2^2 - 3 \leq 0 \}.
\end{align}
Regarding \ref{step:step0} of the proposed synthesis method, a small circle centered at the
origin is considered the initial guess for the DTCBF $h$, i.e.,
\begin{align} \label{eq:sec6:initial-guess}
    h^{(0)} \defeq - x_1^2 - x_2^2 + 0.1. 
\end{align}
Additionally, we utilize $\Lambda \defeq [1 \hspace{0.15cm} x_1 \hspace{0.15cm}x_2 \hspace{0.15cm}x_1x_2 \hspace{0.15cm}x_1^2 \hspace{0.15cm}x_2^2]^{\T}$ as the vector of basis polynomials for the DTCBF parameterized as \eqref{eq:sec4:parameterized-DTCBF} and $\Pi_1 \defeq \Pi_2 \defeq [1 \hspace{0.15cm}x_1 \hspace{0.15cm}x_2]^{\T}$ as the vectors of basis polynomials for the control policy parameterized as \eqref{eq:sec4:parameterized-control-policy}. \\
Regarding function $\gamma(x) \defeq \gamma_0x$, where $\gamma_0 \in (0,1] \subset \mathbb{R}$, assume that we aim to find $\gamma_0$ as closest as possible to $0.5$. This is set as the objective of the problem \eqref{eq:step1:opti1}. \\
The result of the proposed synthesis method is depicted in Figure \ref{fig:sec6:example-linear}. After around $60$ iterations, with each iteration taking average time of $\unit[1.9]{s}$, the DTCBF, the corresponding control policy, and $\gamma$ are synthesized as
\begin{align}
    h(x) &\defeq -0.16x_1^2 - 0.069x_1x_2 - 0.066x_2^2 + 0.16, \nonumber \\
    \pi_1(x) &\defeq \pi_2(x) \defeq -2.31x_1 - 1.02x_2. \nonumber \\
    \gamma(x) &\defeq 0.5x. \nonumber 
\end{align}

\begin{figure}[ht]\centering 
\includegraphics[width=0.45\textwidth]{SOS-CBF/Figures/example-linear-400.png}
    \caption{The proposed synthesis method is applied to the discrete-time system \eqref{eq:sec6:linear-system} and the safe set \eqref{eq:sec6:safe-set} (the interior and boundary of the red circle) to iteratively synthesize a DTCBF, starting from the initial guess DTCBF \eqref{eq:sec6:initial-guess} (black circle). Each of these blue curves represents the updated DTCBF during each iteration.}
    \label{fig:sec6:example-linear}
\end{figure}

==> Sections/Section6-Ex1.tex <==
%\vspace{-0.2cm}
Consider the linearized and discretized cart-pole system discussed in \cite{wu2023neural} as

\begin{align} \label{eq:sec6:linear-system}
    \begin{bmatrix}
        x_c^+ \\ v_c^+ \\ \theta^+ \\ \omega^+
    \end{bmatrix} = \begin{bmatrix}
        0 & 1 & 0 & 0 \\
        0 & 0 & -0.98 & 0 \\
        0 & 0 & 0 & 1 \\
        0 & 0 & 10.78 & 0
    \end{bmatrix}\begin{bmatrix}
        x_c \\ v_c \\ \theta \\ \omega
    \end{bmatrix} + \begin{bmatrix}
        0 \\ 1 \\ 0 \\ -1
    \end{bmatrix}u,
\end{align}
where $x_c, v_c \in \mathbb{R}$ are the horizontal position and velocity of the cart, respectively, $\theta \in \mathbb{R}$ is the angle of the pole from the upward vertical direction, and $\omega \in \mathbb{R}$ is the angular velocity of the pole. Additionally, $x \defeq [x_c ~ v_c ~ \theta ~ \omega]^{\T}$, and \mbox{$u \in \mathbb{U} \defeq [-5, ~ 5]$} is the horizontal force applied to the cart, which is considered as the control input to the system \eqref{eq:sec6:linear-system}. The safe set $\mathcal{S}$ is defined as the disk
\begin{align} \label{eq:sec6:cart-pole-safe-set}
    \mathcal{S} \defeq \{ x \in \mathbb{R}^4 \mid \theta^2 + \omega^2  \leqslant (\pi/5)^2 \}.
\end{align}
We aim to apply our proposed method to synthesize a DTCBF-triple $(h, \gamma, \pi)$ for the system \eqref{eq:sec6:linear-system} with the control admissible set $\mathbb{U}$ and the safe set \eqref{eq:sec6:cart-pole-safe-set} according to the objectives of \mbox{Problem \ref{prob:sec3:synthesis}}. For the initialization step of the proposed synthesis method (Step \ref{step:step0}), a relatively small circle, defined as %\vspace{-0.2cm}
\begin{align} \label{eq:sec6:cart-pole-initial-guess}
    h^{(0)}(x) \defeq - \theta^2 - \omega^2 + 0.04,
\end{align}
is considered as an initial DTCBF. Moreover, we use a vector of monomials up to degrees two and three for the DTCBF $h$ and the control policy $\pi$, parameterized as in \eqref{eq:sec4:parameterized-DTCBF-general} and \eqref{eq:sec4:parameterized-control-policy}, respectively. Regarding $\gamma \in \mathcal{K}^{\leqslant \mathrm{id}}_{\infty}$, we parameterize it as in \eqref{eq:sec4:parameterized-gamma}, and assume that we aim to find $\gamma_0$ as close as possible to $0.8$, which is introduced as an objective in the SOS programming problem \eqref{eq:step1:opti1}.
%as $\gamma(r) \defeq \gamma_0r$, $r \in \mathbb{R}_{\geqslant 0}$ with parameter $\gamma_0 \in (0,1] \subset \mathbb{R}$ unknown, and assume that we aim to find $\gamma_0$ as close as possible to $0.8$. This is set as the objective of the optimization \mbox{problem \eqref{eq:step1:opti1}}. \\
The application of the proposed synthesis method results in \mbox{Figure \ref{fig:sec6:example-cart-pole}}. After around 55 iterations, each taking an average time of $\unit[15]{s}$ (total time about $\unit[14]{min}$), the DTCBF-triple $(h, \gamma, \pi)$ is synthesized as %the DTCBF $h$, the corresponding control policy $\pi$, and $\gamma$ are synthesized as
\begin{align}
    %h(x) &\defeq  - 0.8088\theta^2 - 0.8086\omega^2 + 0.2109, \nonumber \\
    %\pi(x) &\defeq - 1.013\theta^3 + 0.770 \theta \omega^2 + 10.054\theta, \nonumber \\
    h(x) &\defeq  - 1.1706\theta^2 - 1.1715\omega^2 + 0.3032, \nonumber \\
    \pi(x) &\defeq -0.964\theta^3 + 0.701 \theta \omega^2 + 10.074\theta, \nonumber \\
    \gamma(r) &\defeq 0.8r, \quad r \in \mathbb{R}_{\geqslant 0}. \nonumber 
\end{align} %\\[-0.5cm]
It is noteworthy that the synthesized DTCBF $h$ and its friend $\pi$ are independent of $x_c$ and $v_c$. The synthesized DTCBF is depicted in Figure \ref{fig:sec6:example-cart-pole}. To illustrate the level of conservatism in the proposed method for this numerical case study, we also plot the maximal polyhedral controlled invariant set for the system \eqref{eq:sec6:linear-system} with $\mathbb{U}$ using the MPT3 toolbox \cite{MPT3}, without considering \mbox{the safe set $\mathcal{S}$} since it cannot be defined within this toolbox. Specifically, the MPT3 toolbox computes the maximal polyhedral controlled invariant sets for linear systems considering polyhedral state and input constraints. It can be observed that our proposed method synthesizes the quadratic DTCBF with the maximal zero-superlevel set for the system \eqref{eq:sec6:linear-system} with $\mathbb{U}$.

%The zero-superlevel set of the DTCBF $h$ cannot be further expanded in general (not as a limitation of our proposed method) due to the restrictiveness of the control admissible set $\mathbb{U}$. To illustrate this more clearly, we also plot the maximal polyhedral controlled invariant set in Figure \ref{fig:sec6:example-cart-pole} for the system \eqref{eq:sec6:linear-system} with $\mathbb{U}$ using the MPT3 toolbox \cite{MPT3}, without considering the safe set $\mathcal{S}$ (as it cannot be defined in this toolbox). Specifically, the MPT3 toolbox computes the maximal polyhedral controlled invariant sets for linear systems considering polyhedral state and input constraints.
%Moreover, as shown in Figure \ref{fig:sec6:example-cart-pole}, the zero-superlevel set of the \mbox{DTCBF $h$} cannot be further expanded to encompass a larger area within the safe set $\mathcal{S}$. This is due to the restrictiveness of the control admissible set $\mathbb{U}$. 
%diminishes before it reaches the boundary of the safe set $\mathcal{S}$, and eventually it cannot be further enlarged. This is due to the restrictiveness of the control admissible set $\mathbb{U}$.
\begin{figure}[!ht]\centering 
\includegraphics[width=0.43\textwidth]{Figures/cart-pole-grid3.png}
    \caption{The proposed synthesis method is applied to the system \eqref{eq:sec6:linear-system} with the control admissible set $\mathbb{U}$ and the \mbox{safe set \eqref{eq:sec6:cart-pole-safe-set}} (the interior and boundary of the red circle) to iteratively synthesize a DTCBF-triple, starting from the initial DTCBF \eqref{eq:sec6:cart-pole-initial-guess} (black circle). Each of these blue curves represents the updated DTCBF after each iteration. The pale orange square represents the maximal polyhedral controlled invariant set obtained using the MPT3 toolbox \cite{MPT3}.}
    \label{fig:sec6:example-cart-pole}
\end{figure}

